An improved air entrainment model for stepped spillways

Numerical modelling of flow in stepped spillways is considered, focusing on a highly economical approach combining interface capturing with explicit modelling of air entrainment. Simulations are performed on spillways at four different Froude numbers, with flow parameters selected to match available experimental data. First, experiments using the model developed by Lopes et al. (Int. J. Nonlin. Sci. Num., 2017) are conducted. An extensive simulation campaign is used to carefully evaluate the predictive accuracy of the model, the influence of various model parameters, and sensitivity to grid resolution. Results reveal that, at least for the case of stepped spillways, the number of parameters governing the model can be reduced. A crucial identified deficiency of the model is its sensitivity to grid resolution. To improve the performance of the model in this respect, modifications are proposed for the interface detection algorithm and the transport equation for the volume fraction of entrained air. Simulations using the improved model formulation demonstrate better agreement with reference data for all considered flow conditions. A parameter-free criterion for predicting the inception point of air entrainment is also tested. Unfortunately, the accuracy of the considered conventional turbulence models proved to be insufficient for the criterion to work reliably.

==> texfiles/aifbba.tex <==
%%%% AIF bba-sensitivity testing
%% \subsection{Sensitivity on bubble breakup criteria (BBA)}
%% \label{sec:bba}
A bubble breakup criteria is incorporated in the original model. The meaning of
this feature is not to entrain air at locations that are basically in the
continues air phase. By default, this value is set to 0.1, which means that the
air entrainment model is deactivated when the volume fraction of air exceeds
0.9.

In this section the effect of this parameter is explored.

According to %% Table \ref{tab:icpt_bba} and
Figure \ref{fig:h90_bba_dx0025}
turning off the bubble breakup feature has no effect on the prediction of the
inception point and limited effect on the predicted surface height. The void
fraction profiles in Figure \ref{fig:bbacomp_dx0025_alpha} indicates that some
more air is entrained close to the $h_{90}$ surface, by turning off the bubble
breakup model. Compared to the experimental data, it seems to be an overal
tendency that the air fractions predicted by airInterFoam close to the interface
(from $y/h_{90}\approx 0.8$) are too low. By deactivating the bba-criteria, the
results are not much affected, but at least they changes in the direction of
their experimental counterparts (see Figure
\ref{fig:bbacomp_dx0025_alpha}). This might indicate that the bba-criteria does
not make the model better, and could be left out it.



%% \begin{table}[htp]
%%   \caption{Inception points found in \texttt{airInterFoam} (AIF) simulations
%%     compared to physical model results by \cite{Bung2011}.} 
%%   \label{tab:icpt_bba}
%%   \begin{tabular}{llllllll} %{llllll}
%%     \textbf{\textsf{F\textsubscript{s}}} & \textbf{Grid} ($\Delta x$ (m)) &
%%     BBA (-) &
%%     $n_{i,sim}$ & $n_{i,expr}$ & $L_{i,sim}$ & $L_{i,expr}$ & $\Delta
%%     L_{i,expr}$  \\
%%     %% \hline
%%     %% 2.7  & 0.005 & 0.1  & 7  & 5  & 0.94  & 0.67  \\ % case fs27_AIF_dx005_kc02_11692522
%%     %% 2.7  & 0.005 & 0.05 & 7  & 5  & 0.94  & 0.67  \\ % case 
%%     %% 2.7  & 0.005 & 0    & 7  & 5  & 0.94  & 0.67  \\ % case 
%%     \hline
%%     2.7  & 0.0025 & 0.1  & 5.5  & 5  & 0.74  & 0.67 & 0.07  \\ % case 
%%     2.7  & 0.0025 & 0.05 & 5.5  & 5  & 0.74  & 0.67 & 0.07  \\ % case 
%%     2.7  & 0.0025 & 0    & 5.5  & 5  & 0.74  & 0.67 & 0.07  \\ % case 
%%     \hline
%%   \end{tabular}
%% \end{table}




%% %%%% dx=0.0025

%% %%%% Surface elevation plot
%% %% Ur-comp, dx=0.0025
%% \begin{figure}[htp]
%%    \centering
%%    \includegraphics[scale=1,trim={0 0 0 0},clip]{figures/h90_fs27_bbacomp_dx0025.pdf}
%%    \caption{Surface elevation plots. Spillway flows with Froude
%%      number \textsf{F\textsubscript{s}}=2.7, grid resolution $\Delta x=0.0025$
%%      m, and sensitivity on BBA, compared to physical model results
%%      by \cite{Bung2011}.}\label{fig:h90_bba_dx0025} 
%% \end{figure}


%% %%%% Alpha profiles, dx=0.0025
%% \begin{figure}[htp]
%%    \vspace{-8pt}
%%    \centering
%%       \subcaptionbox{Step 7\label{subfig:bbaComp_dx0025_alpha_M7}}
%%         {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs27_bbacomp_dx0025_M7.pdf}}
%%       \subcaptionbox{Step 11\label{subfig:bbaComp_dx0025_alpha_M11}}
%%         {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs27_bbacomp_dx0025_M11.pdf}}
%%       \subcaptionbox{Step 15\label{subfig:bbaComp_dx0025_alpha_M15}}
%%         {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
%%               3},clip]{figures/alpha_fs27_bbacomp_dx0025_M15.pdf}}
%%       \subcaptionbox{Step 19\label{subfig:bbaComp_dx0025_alpha_M19}}
%%         {\includegraphics[scale=1,trim={0.7cm 10 0
%%               3},clip]{figures/alpha_fs27_bbacomp_dx0025_M19.pdf}}
        
%%         \caption{Vertical void fraction profiles for different step niches in
%%           the development region. Spillway flows with Froude number
%%           \textsf{F\textsubscript{s}}=2.7, grid resolution $\Delta x=0.0025$ m,
%%           and with sensitivity on BBA, compared to physical model
%%           results by \cite{Bung2011}. }\label{fig:bbacomp_dx0025_alpha} 
%% \end{figure}



==> texfiles/aifdiff.tex <==
%%%% AIF - sensitivity on diffusion
\subsection{Sensitivity on diffusion}
\label{sec:aifdiff}
To assist in distributing the entrained air away from the surface a diffusion
term can be activated in the $\alpha_g$-equation (Equation
(\ref{eq:alphag})). As outlined in Section \ref{subsec:alphag} this term can be
activated as an user input boolean. Nevertheless, according to the results shown
in Figure \ref{fig:h90_diffaif_dx0025} and \ref{fig:diffaif_dx0025_alpha}, the
influence of activating this term seems to be negligible.   



%% %%%% Surface elevation plot
%% %% diffusion-comp, dx=0.0025
%% \begin{figure}[htp]
%%    \centering
%%    \includegraphics[scale=1,trim={0 0 0 0},clip]{figures/h90_fs27_diffaif_dx0025.pdf}
%%    \caption{Surface elevation plots. Spillway flows with Froude
%%      number \textsf{F\textsubscript{s}}=2.7, grid resolution $\Delta x=0.0025$
%%      m, and sensitivity on diffusion, compared to physical model results
%%      by \cite{Bung2011}.}\label{fig:h90_diffaif_dx0025} 
%% \end{figure}

%% %%%% Alpha profiles, dx=0.0025
%% \begin{figure}[htp]
%%    \vspace{-8pt}
%%    \centering
%%       %% \subcaptionbox{Step 7\label{diffaif_dx0025_alpha_M7}}
%%       %%   {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs27_diffaif_dx0025_M7.pdf}}
%%       %% \subcaptionbox{Step 11\label{diffaif_dx0025_alpha_M11}}
%%       %%   {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs27_diffaif_dx0025_M11.pdf}}
%%       %% \subcaptionbox{Step 15\label{diffaif_dx0025_alpha_M15}}
%%       %%   {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
%%       %%         3},clip]{figures/alpha_fs27_diffaif_dx0025_M15.pdf}}
%%       \subcaptionbox{Step 19\label{diffaif_dx0025_alpha_M19}}
%%         {\includegraphics[scale=1,trim={0.7cm 10 0
%%               3},clip]{figures/alpha_fs27_diffaif_dx0025_M19.pdf}}
        
%%         \caption{Vertical void fraction profiles for step 19 (uniform
%%           region). Spillway flows with Froude number
%%           \textsf{F\textsubscript{s}}=2.7, grid resolution $\Delta x=0.0025$ m,
%%           and with sensitivity on diffusion, compared to physical model
%%           results by \cite{Bung2011}. }\label{fig:diffaif_dx0025_alpha} 
%% \end{figure}



==> texfiles/aifkccomp.tex <==
\subsection{Sensitivity to $k_c$}
\label{sec:aifkc}

Recall that the \textsf{F\textsubscript{s}}-sensitivity study revealed that the predictions of the inception point deteriorate with increasing \textsf{F\textsubscript{s}}.
This prompts using a different value of $k_c$ for these cases, and it is therefore interesting to see how sensitive the inception point location is with respect to the prescribed value.


%As shown in Table \ref{tab:aifkc}, the inception points predicted using the
%default $k_c$-value of 0.2, gives relatively good accuracy for
%\textsf{F\textsubscript{s}}=2.7 and \textsf{F\textsubscript{s}}=8.3, which are
%the low discharge cases. For \textsf{F\textsubscript{s}}=4.6 and
%\textsf{F\textsubscript{s}}=13, the deviation from the experimental values are
%relatively large. Further, the inception point is
%predicted earlier for \textsf{F\textsubscript{s}}=13, then for
%\textsf{F\textsubscript{s}}=8.3, which contradicts both the experimental data
%and theory, and indicates that $k_c$ should be a function of the
%discharge. \textcolor{red}{Perhaps write some sort of description of the
%  physics involved in the balance of forces here...}
%Changing $k_c$ to 0.3 for the high discharge cases \textsf{F\textsubscript{s}}=4.6
%and \textsf{F\textsubscript{s}}=13, substantially improves the prediction of
%the inception point for \textsf{F\textsubscript{s}}=13. The deviation from the
%corresponding experimental result were reduced for the \textsf{F\textsubscript{s}}=4.6
%case as well, but the inception point were now predicted too far downstream, instead of
%too far upstream, which was the case using $k_c=0.2$. Based on this a
%$k_c$-value between 0.2 and 0.3 might be appropriate for this case. These
%results might indicate that the value of $k_c$ should be a function of discharge
%and step size.


\begin{table}[htp]
  \begin{minipage}{.5\textwidth}
  \caption{Inception points obtained with AIF simulations for
    \textsf{F\textsubscript{s}}=2.7, grid resolution G3, and different input
    values of the critical kinetic energy, $k_c$, compared to physical model
    results by \citet{Bung2011}. \textcolor{red}{Hmmm...a bit unsure about this,
  the results using G1 is quite different from G3, like 50\% change, and the
  change is a bit differnet from case to case...at G1 it is fs8.2 and fs13 that
  is worth, so did that here...for now at least... Might also be interesting to
  show how this changes with grid resolution...? Have to rewrite the text after
  decided what to do...}}
  \label{tab:aifkc}
  \begin{tabular}{lllllllll} %{llllll}
    \textsf{F\textsubscript{s}} & \textbf{Grid} & \textbf{$k_c$}  &

    $L_{i,sim}$ & $L_{i,expr}$ & $\Delta L_i$ & $\Delta n_i$ \\
    \hline
    2.7  & G1  &  0.2   & 0.94  & 0.67 & 0.27 & 2 \\ % case fs27_AIF_dx00125_kc02_786650
    4.6  & G1  &  0.2   & 1.14 & 0.95  & 0.19 & 1 \\ % case fs46_AIF_dx00125_kc02_786670
    8.3  & G1  &  0.2   & 1.71 & 1.14  &  0.57 & 6   \\ % case
    13   & G1  &  0.2   & 1.43 & 2.0   & -0.57 & -6  \\ % case
    \hline
    8.3  & G1  &  0.1  & 0.76  & 1.14 &  -0.38 & -4 \\ % case
    13   & G1  &  0.3  & 2.57  & 2.0  & 0.57  & 6  \\ % case
    \hline
  \end{tabular}
  \end{minipage}
\end{table}


==> texfiles/aifturbcomp.tex <==
%%%% Comparison of different turbulence models
\subsection{Sensitivity on turbulence model}
\label{sec:aifturbmod}
The air entrainment model (Equation (\ref{eq:sg}),(\ref{eq:a}),(\ref{eq:kc}))   
rely on the calculated turbulence fields, which implies that the turbulence
calculations are of substantial importance for the result. In this sequence the
behavior of 
$k \omega$ and realizable-$k \eps$ turbulence models is explored on the two
finest grids (G3 and G4). These models
have been tested with the standard OpenFOAM turbulence framework, and with the
variable density framework by \citet{Fan2020}.


From initial inception point calibration towards the experimental data on grid
G2 using the variable density turbulence framework, 0.03 was found as a
proper value for $k_c$. The corresponding 
value using the standard OpenFOAM turbulence framework was $k_c=0.2$, which is
about one order of magnitude 
higher.
%% Even if this might stand as a result on its own, this section
%% gives a comparison of the overall behaviour of the different turbulence models,
%% using $k_c$-values individually calibrated for the different turbulence
%% frameworks.


\begin{table}[htp]
  \begin{minipage}{.55\textwidth}
  \caption{Inception points found in \texttt{airInterFoam} (AIF) simulations
    at grid G3 and G4, using different models for turbulence modelling,
    compared to physical model results by \citet{Bung2011}.} 
  \label{tab:turb}
  \begin{tabular}{llllrr} %{ccccccc} %{llllll}
    \textbf{\textsf{F\textsubscript{s}}} & \textbf{Grid} & \textbf{Turbulence} &
    \textbf{$k_c$} & $\Delta n_{i,expr}$  & $\Delta L_{i,expr}$\\
    \hline
    2.7  & G3 & $k\omega$              & 0.20 & -0.5 & -0.07 \\ % case 786650
    2.7  & G3 & rKE                    & 0.20 & -0.5 & -0.07 \\ % case 11750456
    2.7  & G3 & \ttt{varRho}/$k\omega$ & 0.03 & 1.5  & 0.20 \\ % case 786650
    2.7  & G3 & \ttt{varRho}/rKE       & 0.03 & 1    & 0.13 \\ % case 11795631
    \hline
    2.7  & G4 & $k\omega$              & 0.20 & -1.5 & -0.20  \\ % case 
    2.7  & G4 & rKE                    & 0.20 & -0.5 & -0.07 \\ % case
    2.7  & G4 & \ttt{varRho}/$k\omega$ & 0.03 & 3.5  &  0.47 \\ % case 786650
    2.7  & G4 & \ttt{varRho}/rKE       & 0.03 & 2    &  0.27 \\ % case
    \hline
  \end{tabular}
  \end{minipage}
\end{table}

The qualitative behavior seems to be similar for the different turbulence
models (see Figure \ref{fig:h90_turbComp_dx0625}). However, at this grid
resolution the model does not entrain much air (see Figure
\ref{subfig:alphaField_fs13_G4_grid}), which means 
that the model does not work very well. As illustrated by the surface elevation
plot in Figure \ref{fig:h90_turbComp_dx0625}, applying the
realizable $k\eps$-model for the standard turbulence framework, some more air was
entrained. This was also reflected by void fraction profiles and velocity curves
(not shown). Nevertheless, similar behaviour was not seen for corresponding
simulations using the variable density framework.

A thing that might be worth noting is that using the variable density framework,
the inception point tends to be predicted further downstream as the cell density
increases, while using the standard turbulence framework, the inception point
tends to be predicted further upstream by grid refinement. According to Table
\ref{tab:turb}, the realizable $k \eps$ model tends to show a more grid
convergent solution in terms of inception point variation between the grids in
question. 


%%%% dx=0.000625 %%%%

%% %%%% Alpha field plot
%% % Sensitivity on turbulence model -- dx=0.000625
%% \begin{figure}[htp]
%%    \centering
%%     \begin{subfigure}[b]{\textwidth}
%%         \includegraphics[scale=1,trim={0 10 0 0},clip]{figures/alphaField_fs27_kOm_dx000625}
%%         \caption{$k \omega$}
%%         \label{subfig:alphaField_fs27_kOm_dx000625}
%%     \end{subfigure}
%%     %% \bigskip
%%     \par\medskip
%%      %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%%       %(or a blank line to force the subfigure onto a new line)
%%     \begin{subfigure}[b]{\textwidth}
%%         \includegraphics[scale=1,trim={0 10 0 0},clip]{figures/alphaField_fs27_rke_dx000625}
%%         \caption{realizable $k \epsilon$}
%%         \label{subfig:alphaField_fs46_rke_dx000625}
%%     \end{subfigure}
%%     \par\medskip
%%      %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%%     %(or a blank line to force the subfigure onto a new line)
%%     \begin{subfigure}[b]{\textwidth}
%%         \includegraphics[scale=1,trim={0 10 0 0},clip]{figures/alphaField_fs27_vrkOm_dx000625}
%%         \caption{\ttt{varRho} -- $k \omega$}
%%         \label{subfig:alphaField_fs82_vrkOm_dx000625}
%%     \end{subfigure}
%%     \par\medskip
%%      %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%%     %(or a blank line to force the subfigure onto a new line)
%%     \begin{subfigure}[b]{\textwidth}
%%         \includegraphics[scale=1,trim={0 10 0 0},clip]{figures/alphaField_fs27_vrrke_dx000625}
%%         \caption{\ttt{varRho} -- realizable $k \epsilon$}
%%         \label{subfig:alphaField_fs82_kc03_dx000625}
%%     \end{subfigure}
%%     \caption{Void fraction field plots. Sensitivity on turbulence model on
%%       spillway flows with Froude number \textsf{F\textsubscript{s}}=2.7. Grid
%%       resolusion $\Delta x = 0.000625$ m.  \textcolor{red}{Perhaps zooming this
%%         figures and place annotations with inception point location, or
%%         difference}}\label{fig:alphaField_turb_dx000625}
%% \end{figure}


%%%% Surface elevation plot
%% turb-comp, dx=0.000625
\begin{figure}[htp]
   \centering
   \includegraphics[scale=1,trim={0 0 0 0},clip]{figures/h90_fs27_turbcomp_dx0625.pdf}
   \caption{Surface elevation plots. Spillway flows with Froude
     number \textsf{F\textsubscript{s}}=2.7, grid resolution G4, and
     different turbulence models, compared to physical model results 
     by \citet{Bung2011}.}\label{fig:h90_turbComp_dx0625} 
\end{figure}


%% %%%% Alpha profiles, dx=0.000625
%% \begin{figure}[htp]
%%    \vspace{-8pt}
%%    \centering

%%       \subcaptionbox{Step 19\label{subfig:turbComp_dx0625_alpha_M19}}
%%         {\includegraphics[scale=1,trim={0.7cm 10 0
%%               3},clip]{figures/alpha_fs27_turbcomp_dx0625_M19.pdf}}
%%      \subcaptionbox{Step 19\label{subfig:turbComp_dx00625_ux_M19}}
%%         {\includegraphics[scale=1,trim={0.7cm 10 0
%%               3},clip]{figures/ux_fs27_turbcomp_dx0625_M19.pdf}}        
%%         \caption{Vertical velocity and void fraction profiles for 
%%           the uniform region. Spillway flows with Froude number
%%           \textsf{F\textsubscript{s}}=2.7, grid resolution $\Delta x=0.000625$ m,
%%           and with different turbulence models, compared to physical model
%%           results by \cite{Bung2011}. }\label{turbComp_dx00625_alpha_ux} 
%% \end{figure}



==> texfiles/applicGuidelines.tex <==
\section{Application guidelines}
\label{sec:appguidelines}
The developed model \ttt{spillwayFlow} contains several parameters available for
the user as input variables. In the following subsections, guidance on how
to set these variables are given.

\subsection{Diffusion}
It seems like some degree of diffusion is needed to be able to get the air
transported from the surface towards the step pseudo-bottom. In the current work
the constant $C_b$ was added as a factor to the diffusion term. In the reported
results, $C_b=150$ was used for all cases. Nevertheless, the results showed that
perhaps this constant should depent on the step Froude number, step height or
the discharge. The usefulness of the diffusion term might also depend on the
application. In terms of surface height, results tended to be better represented
omitting the diffusion term.

\subsection{Interface thickness}
The interface thickness is supposed to reflect the surface thickness introduced
by the roughening of the free surface, and should imitate the thickness of the
region where air might be entrained. As indicated by \citet{Ma2011}, this
parameter should be chosen to depend on some characteristic length of the
problem. For the simulations in this work, the interface thickness were set
equal to $\phi_{ent}$ and $0.05L$, where $h_c$ was chosen as the characteristic
length $L$. (\textcolor{red}{see Lopes reference on this to explore it a little
  more}).     
Compined with the diffusion constant $C_b=150$, this seemed to produced results
of reasonable accuracy for tested stepped spillway cases. In terms of
reproducing the surface height, the results in Section
\ref{subsec:spf_difftesting} indicates that an equivalent air depth $h_{air}$,
might be an useful value for the interface thickness. 

\subsection{$u_{cr}$}
This variable was not used. \textcolor{red}{Perhaps we should remove this
  parameter from the solver...?}

\subsection{Delta function cutoff}
This parameter is described in Section \ref{subsec:fsdetection}, and denotes the
cutoff value for $\nabla \alpha_l$ . In the current work a value of 20 was found
as a proper value for this parameter, and used in all simulation cases. If this
value are set too high, too litle air is introduced, and if set too zero, one
will not get a gradual reduction in air entrainment away from tha surface within
the surface region. \textcolor{red}{Or perhaps this parameter should be
  hardcoded...?}

\subsection{nCriticalGrad}
This parameter denotes how many cells a interface should be over to be defined
as a sharp interface, and is described in Section \ref{subsec:fsdetection}. In
this work the philosophy for this variable is to set it tight. In that way we
use $|\nabla \alpha_l|_{crit}$ to identify a sharp interface, as a reference to
decide on the interface thickness. Then we broaden the sharp interface into a
interface region by setting $\nabla \alpha_{l,\text{cutOff}}$ considerably
lower.

\subsection{$k_c$}
The critical kinetic energy criteria used in \ttt{airInterFoam} is left as an
option to be used for the onset of air entrainment. By setting this parameter to
zero, the activation criteria given in Equation (\ref{eq:ptpd}) will be used. If
$k_c$ are used as the onset criteria, it should be taken into account that
a decent value for this parameter seems to depend on the discharge, or some
characteristic scale of the problem.  


==> texfiles/notation.tex <==
\section*{Notation}
%% An unnumbered `Notation' section, e.g. \verb"\section*{Notation}", should include the main variables used in the paper in alphabetical order with Latin symbols given first, followed by Greek symbols (with no subheadings). The SI units should be given for each variable (if relevant) in round brackets in regular Times New Roman font, e.g.:\\

\begin{tabular}{@{}ll}
  \textsf{F} & = Froude number (--)\\
  \textsf{F\textsubscript{s}} & = step Froude number (--)\\
$g$ & = gravity acceleration (m s$^{-2}$) \\
\textsf{R\textsubscript{e}} & = Reynolds number (--)\\
\end{tabular}\\


==> texfiles/publication.tex <==
\section*{Possible journals}
\begin{itemize}
\item water
  \begin{itemize}
    \item Open access journal - charge of $\approx$ 18000 SEK
  \end{itemize}
\item Applied Mathematical Modelling
  \begin{itemize}
  \item https://www.journals.elsevier.com/applied-mathematical-modelling
  \item Published Lopes' first paper \cite{Lopes2016}
  \item \textit{Applied Mathematical Modelling focuses on research related to the
    mathematical modelling of engineering and environmental processes,
    manufacturing, and industrial systems.}
    \item Free of charge
  \end{itemize}
\item Journal of Fluids Engineering
  \begin{itemize}
  \item Chanson have published papers here
    \item Crappy homepage 
  \end{itemize}
\item Journal of Hydraulic Engineering
  \begin{itemize}
  \item Not open access -- perhaps an alternative...?
  \item Allows latex
    \item \textit{For most ASCE journals, the maximum length for technical papers and
      case studies is 30 double-spaced manuscript pages including references,
      figures, tables, and captions}
    \item Crappy homepage
      \item Impact factor 2.2 (2018)
  \end{itemize}
\item International Journal of Computational Fluid Dynamics
\begin{itemize}
  \item There are no submission fees, publication fees or page charges for this
    journal
\end{itemize}
\item Engineering Applications of Computational Fluid Mechanics
  \begin{itemize}
  \item Open access journal
  \item My previous publication was here
  \end{itemize}
\item ISH Journal of Hydraulic Engineering
  \begin{itemize}
  \item Not open access
  \item Low impact factor
  \end{itemize}
\end{itemize}


==> texfiles/spflfscomp.tex <==
% fs-comp for spillwayFlow
\subsection{Sensitivity on \textsf{F\textsubscript{s}}}

%%%% Surface elevation plot
%% Could perhaps made this as one plot - have to think about this...
%% dx=0.005
\begin{figure}[htp]
  \vspace{-10pt}
   \centering
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 20 0 0},clip]{figures/h90_fs27_gridcomp_spf.pdf}
        \caption{\textsf{F\textsubscript{s}}=2.7}
        \label{subfig:h90_fs27_dx005}
    \end{subfigure}
    %% \bigskip
    \par\medskip
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 20 0 20},clip]{figures/h90_fs46_gridcomp_spf_noLegend.pdf}
        \caption{\textsf{F\textsubscript{s}}=4.6}
        \label{subfig:h90_fs46_dx005}
    \end{subfigure}
    \par\medskip
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 20 0 20},clip]{figures/h90_fs82_gridcomp_spf_noLegend.pdf}
        \caption{\textsf{F\textsubscript{s}}=8.28}
        \label{subfig:h90_fs82_dx005}
    \end{subfigure}
    \par\medskip
        \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 10 0 20},clip]{figures/h90_fs13_gridcomp_spf_noLegend.pdf}
        \caption{\textsf{F\textsubscript{s}}=13}
        \label{subfig:h90_fs13_dx005}
    \end{subfigure}
    \caption{Surface elevation plots. Spillway flows with different Froude
      numbers on the coarsest grid ($\Delta x=0.005$ m, $\approx 100 000$ cells)
      compared to physical model results by
      \cite{Bung2011}.}\label{fig:h90_fscomp_dx005} 
\end{figure}


%%%% Alpha profiles

%% All included
%% Steg edges
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
      % dx=0.005
      \subcaptionbox{\textsf{F\textsubscript{s}}=2.7  \label{subfig:fs27_alpha}}
        {\includegraphics[scale=1,trim={0.3cm 20 0 0},clip]{figures/alpha_fs27_gridcomp_spf_M19_legend.pdf}}
        %\hfill
      \subcaptionbox{\textsf{F\textsubscript{s}}=4.6\label{subfig:fs46_alpha}}
                    {\includegraphics[scale=1,trim={0.8cm 20 0 0},clip]{figures/alpha_fs46_gridcomp_spf_M19.pdf}}
      \subcaptionbox{\textsf{F\textsubscript{s}}=8.28\label{subfig:fs828_alpha}}
        {\includegraphics[scale=1,trim={0.8cm 20 0
              0},clip]{figures/alpha_fs82_gridcomp_spf_E32.pdf}}
      \subcaptionbox{\textsf{F\textsubscript{s}}=13\label{subfig:fs13_alpha}}
        {\includegraphics[scale=1,trim={0.8cm 20 0
              0},clip]{figures/alpha_fs13_gridcomp_spf_E38.pdf}}
        \\
        \caption{Vertical void fraction profiles for uniform flow
          conditions. Spillway flows with different Froude numbers
          computed at the two finest grid ($\Delta x=0.00125$ m $\approx
          1.4-1.9$ million cells, $\Delta x=0.000625$ m $\approx 5-7$ million
          cells). Simulation results from SPF and AIF compared to physical model
          results by \cite{Bung2011}.}\label{fig:fsComp_alpha_dx005}
\end{figure}

%% Steg niches (for fs27 and fs46)
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
      % dx=0.005
      \subcaptionbox{\textsf{F\textsubscript{s}}=2.7  \label{subfig:fs27_alpha_spfE}}
        {\includegraphics[scale=1,trim={0.3cm 20 0 0},clip]{figures/alpha_fs27_gridcomp_spf_E19_legend.pdf}}
        %\hfill
      \subcaptionbox{\textsf{F\textsubscript{s}}=4.6\label{subfig:fs46_alpha_spfE}}
                    {\includegraphics[scale=1,trim={0.8cm 20 0 0},clip]{figures/alpha_fs46_gridcomp_spf_E19.pdf}}
      \subcaptionbox{\textsf{F\textsubscript{s}}=8.28\label{subfig:fs828_alpha_spfE}}
        {\includegraphics[scale=1,trim={0.8cm 20 0
              0},clip]{figures/alpha_fs82_gridcomp_spf_E32.pdf}}
      \subcaptionbox{\textsf{F\textsubscript{s}}=13\label{subfig:fs13_alpha_spfE}}
        {\includegraphics[scale=1,trim={0.8cm 20 0
              0},clip]{figures/alpha_fs13_gridcomp_spf_E38.pdf}}
        \\
        \caption{Vertical void fraction profiles for uniform flow
          conditions. Spillway flows with different Froude numbers
          computed at the two finest grid ($\Delta x=0.00125$ m $\approx
          1.4-1.9$ million cells, $\Delta x=0.000625$ m $\approx 5-7$ million
          cells). Simulation results from SPF and AIF compared to physical model
          results by \cite{Bung2011}. Profiles from step edges for all
          cases.}\label{fig:fsComp_alpha_dx005} 
\end{figure}


%% Velocity profiles
\begin{figure}[htp]
%  \vspace{-100pt}
  \centering

  %% dx=0.005 
      \subcaptionbox{\textsf{F\textsubscript{s}}=2.7\label{spf_fs27_vel}}
        {\includegraphics[scale=1,trim={0.3cm 10 0 0},clip]{figures/ux_fs27_gridcomp_spf_M19_legend.pdf}}
        %\hfill
      \subcaptionbox{\textsf{F\textsubscript{s}}=4.6\label{spf_fs46_vel}}
                    {\includegraphics[scale=1,trim={0.8cm 10 0 0},clip]{figures/ux_fs46_gridcomp_spf_M19.pdf}}
      \subcaptionbox{\textsf{F\textsubscript{s}}=8.28\label{spf_fs828_vel}}
        {\includegraphics[scale=1,trim={0.8cm 10 0
              0},clip]{figures/ux_fs82_gridcomp_spf_E32.pdf}}
        \subcaptionbox{\textsf{F\textsubscript{s}}=13\label{spf_fs13_vel}}
        {\includegraphics[scale=1,trim={0.8cm 10 0
              0},clip]{figures/ux_fs13_gridcomp_spf_E38.pdf}} \\
        \caption{Vertical velocity profiles for uniform flow
          conditions. Spillway flows with different Froude numbers
          on the coarsest grid ($\Delta x=0.005$ m, $\approx 100 000$
          cells) compared to physical model results by
          \cite{Bung2011}. }\label{spf_fsComp_vel}
\end{figure}


==> texfiles/spflgridcomp.tex <==
%% final grid comp
\subsection{Grid sensitivity}

%%%% fs = 2.7
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Surface elevation plot
\begin{figure}[htp]
   \centering
   \includegraphics[scale=1,trim={0 0 0 0},clip]{figures/h90_fs27_gridcomp_spf.pdf}
   \caption{Surface elevation plots. Spillway flows with Froude
     number\textsf{F\textsubscript{s}}=2.7 SPF for grid G3 and G4, and
     corresponding simulations for AIF, compared to
     physical model results by \cite{Bung2011}.}\label{fig:h90_fscomp_spf}
\end{figure}

%%%% Alpha profiles -- step niches
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
        %dx = 0.000625
      \subcaptionbox{Step niche 7\label{subfig:gridComp_alpha_spf_M7}}
        {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs27_gridcomp_spf_M7.pdf}}
      \subcaptionbox{Step niche 11\label{subfig:gridComp_alpha_spf_M11}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs27_gridcomp_spf_M11.pdf}}
      \subcaptionbox{Step niche 15\label{subfig:gridComp_alpha_spf_M15}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/alpha_fs27_gridcomp_spf_M15.pdf}}
      \subcaptionbox{Step niche 19\label{subfig:gridComp_alpha_spf_M19}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/alpha_fs27_gridcomp_spf_M19.pdf}}
        
        \caption{Vertical void fraction profiles for different step niches in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=2.7 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridCompfs27_spf_alpha}
\end{figure}

%%%% Alpha profiles -- step edges
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
        %dx = 0.000625
      \subcaptionbox{Step edge 7\label{subfig:gridComp_alpha_spf_E7}}
        {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs27_gridcomp_spf_E7.pdf}}
      \subcaptionbox{Step edge 11\label{subfig:gridComp_alpha_spf_E11}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs27_gridcomp_spf_E11.pdf}}
      \subcaptionbox{Step edge 15\label{subfig:gridComp_alpha_spf_E15}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/alpha_fs27_gridcomp_spf_E15.pdf}}
      \subcaptionbox{Step edge 19\label{subfig:gridComp_alpha_spf_E19}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/alpha_fs27_gridcomp_spf_E19.pdf}}
        
        \caption{Vertical void fraction profiles for different step edges in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=2.7 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridComp_spf_alpha}
\end{figure}

%%%% Velocity profiles
\begin{figure}[htp]
%   \vspace{-8pt}
   \centering
        %dx = 0.000625
     \subcaptionbox{Step 7\label{subfig:gridComp_spf_ux_M7}}
        {\includegraphics[scale=1,trim={0 10 0.2cm 3},clip]{figures/ux_fs27_gridcomp_spf_M7.pdf}}
     \subcaptionbox{Step 11\label{subfig:gridComp_spf_ux_M11}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/ux_fs27_gridcomp_spf_M11.pdf}}
     \subcaptionbox{Step 15\label{subfig:gridComp_spf_ux_M15}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/ux_fs27_gridcomp_spf_M15.pdf}}
     \subcaptionbox{Step 19\label{subfig:gridComp_spf_ux_M19}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/ux_fs27_gridcomp_spf_M19.pdf}}
        
        \caption{Vertical velocity profiles for different step niches in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=2.7 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridComp_spf_ux}
\end{figure}


%%%% fs = 4.6
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Surface elevation plot
\begin{figure}[htp]
   \centering
   \includegraphics[scale=1,trim={0 0 0 0},clip]{figures/h90_fs46_gridcomp_spf.pdf}
   \caption{Surface elevation plots. Spillway flows with Froude
     number\textsf{F\textsubscript{s}}=4.6 SPF for grid G3 and G4, and
     corresponding simulations for AIF, compared to
     physical model results by \cite{Bung2011}.}\label{fig:h90_gridcompfs46_spf}
\end{figure}

%%%% Alpha profiles -- step niches
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
        %dx = 0.000625
      \subcaptionbox{Step niche 7\label{subfig:gridCompfs46_alpha_spf_M7}}
        {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs46_gridcomp_spf_M7.pdf}}
      \subcaptionbox{Step niche 11\label{subfig:gridCompfs46_alpha_spf_M11}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs46_gridcomp_spf_M11.pdf}}
      \subcaptionbox{Step niche 15\label{subfig:gridCompfs46_alpha_spf_M15}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/alpha_fs46_gridcomp_spf_M15.pdf}}
      \subcaptionbox{Step niche 19\label{subfig:gridCompfs46_alpha_spf_M19}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/alpha_fs46_gridcomp_spf_M19.pdf}}
        
        \caption{Vertical void fraction profiles for different step niches in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=4.6 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridCompfs46_spf_alpha}
\end{figure}

%%%% Alpha profiles -- step edges
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
        %dx = 0.000625
      \subcaptionbox{Step edge 7\label{subfig:gridCompfs46_alpha_spf_E7}}
        {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs46_gridcomp_spf_E7.pdf}}
      \subcaptionbox{Step edge 11\label{subfig:gridCompfs46_alpha_spf_E11}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs46_gridcomp_spf_E11.pdf}}
      \subcaptionbox{Step edge 15\label{subfig:gridCompfs46_alpha_spf_E15}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/alpha_fs46_gridcomp_spf_E15.pdf}}
      \subcaptionbox{Step edge 19\label{subfig:gridCompfs46_alpha_spf_E19}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/alpha_fs46_gridcomp_spf_E19.pdf}}
        
        \caption{Vertical void fraction profiles for different step edges in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=4.6 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridComp_spf_alpha}
\end{figure}

%%%% Velocity profiles
\begin{figure}[htp]
%   \vspace{-8pt}
   \centering
        %dx = 0.000625
     \subcaptionbox{Step niche 7\label{subfig:gridCompfs46_spf_ux_M7}}
        {\includegraphics[scale=1,trim={0 10 0.2cm 3},clip]{figures/ux_fs46_gridcomp_spf_M7.pdf}}
     \subcaptionbox{Step niche 11\label{subfig:gridCompfs46_spf_ux_M11}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/ux_fs46_gridcomp_spf_M11.pdf}}
     \subcaptionbox{Step niche 15\label{subfig:gridCompfs46_spf_ux_M15}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/ux_fs46_gridcomp_spf_M15.pdf}}
     \subcaptionbox{Step niche 19\label{subfig:gridCompfs46_spf_ux_M19}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/ux_fs46_gridcomp_spf_M19.pdf}}
        \caption{Vertical velocity profiles for different step niches in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=4.6 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridCompfs46_spf_ux}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% fs = 8.28
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Surface elevation plot
\begin{figure}[htp]
   \centering
   \includegraphics[scale=1,trim={0 0 0 0},clip]{figures/h90_fs82_gridcomp_spf.pdf}
   \caption{Surface elevation plots. Spillway flows with Froude
     number\textsf{F\textsubscript{s}}=8.28 SPF for grid G3 and G4, and
     corresponding simulations for AIF, compared to
     physical model results by \cite{Bung2011}.}\label{fig:h90_gridcomp_spf_fs82}
\end{figure}

%%%% Alpha profiles -- step edges
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
        %dx = 0.000625
      \subcaptionbox{Step edge 15\label{subfig:gridCompfs82_alpha_spf_E15}}
        {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs82_gridcomp_spf_E15.pdf}}
      \subcaptionbox{Step edge 20\label{subfig:gridCompfs82_alpha_spf_E20}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs82_gridcomp_spf_E20.pdf}}
      \subcaptionbox{Step edge 27\label{subfig:gridCompfs82_alpha_spf_E27}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/alpha_fs82_gridcomp_spf_E27.pdf}}
      \subcaptionbox{Step edge 32\label{subfig:gridCompfs82_alpha_spf_E32}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/alpha_fs82_gridcomp_spf_E32.pdf}}
        
        \caption{Vertical void fraction profiles for different step edges in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=8.28 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridCompfs82_spf_alpha}
\end{figure}

%%%% Velocity profiles
\begin{figure}[htp]
%   \vspace{-8pt}
   \centering
        %dx = 0.000625
     \subcaptionbox{Step 15\label{subfig:gridCompfs82_spf_ux_E15}}
        {\includegraphics[scale=1,trim={0 10 0.2cm 3},clip]{figures/ux_fs82_gridcomp_spf_E15.pdf}}
     \subcaptionbox{Step 20\label{subfig:gridCompfs82_spf_ux_E20}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/ux_fs82_gridcomp_spf_E20.pdf}}
     \subcaptionbox{Step 27\label{subfig:gridCompfs82_spf_ux_E27}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/ux_fs82_gridcomp_spf_E27.pdf}}
     \subcaptionbox{Step 32\label{subfig:gridCompfs82_spf_ux_E32}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/ux_fs82_gridcomp_spf_E32.pdf}}
        \caption{Vertical velocity profiles for different step niches in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=8.28 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridCompfs82_spf_ux}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% fs = 13
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Surface elevation plot
\begin{figure}[htp]
   \centering
   \includegraphics[scale=1,trim={0 0 0 0},clip]{figures/h90_fs13_gridcomp_spf.pdf}
   \caption{Surface elevation plots. Spillway flows with Froude
     number\textsf{F\textsubscript{s}}=13 SPF for grid G3 and G4, and
     corresponding simulations for AIF, compared to
     physical model results by \cite{Bung2011}.}\label{fig:h90_gridcomp_spf_fs82}
\end{figure}

%%%% Alpha profiles -- step edges
\begin{figure}[htp]
   \vspace{-8pt}
   \centering
        %dx = 0.000625
      \subcaptionbox{Step edge 22\label{subfig:gridCompfs13_alpha_spf_E22}}
        {\includegraphics[scale=1,trim={0.1cm 10 0.2cm 3}]{figures/alpha_fs13_gridcomp_spf_E22.pdf}}
      \subcaptionbox{Step edge 26\label{subfig:gridCompfs13_alpha_spf_E26}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/alpha_fs13_gridcomp_spf_E26.pdf}}
      \subcaptionbox{Step edge 33\label{subfig:gridCompfs13_alpha_spf_E33}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/alpha_fs13_gridcomp_spf_E33.pdf}}
      \subcaptionbox{Step edge 38\label{subfig:gridCompfs13_alpha_spf_E38}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/alpha_fs13_gridcomp_spf_E38.pdf}}
        
        \caption{Vertical void fraction profiles for different step edges in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=13 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridCompfs13_spf_alpha}
\end{figure}

%%%% Velocity profiles
\begin{figure}[htp]
%   \vspace{-8pt}
   \centering
        %dx = 0.000625
     \subcaptionbox{Step 15\label{subfig:gridCompfs13_spf_ux_E22}}
        {\includegraphics[scale=1,trim={0 10 0.2cm 3},clip]{figures/ux_fs13_gridcomp_spf_E22.pdf}}
     \subcaptionbox{Step 20\label{subfig:gridCompfs13_spf_ux_E26}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm 3},clip]{figures/ux_fs13_gridcomp_spf_E26.pdf}}
     \subcaptionbox{Step 27\label{subfig:gridCompfs13_spf_ux_E33}}
        {\includegraphics[scale=1,trim={0.7cm 10 0.2cm
              3},clip]{figures/ux_fs13_gridcomp_spf_E33.pdf}}
     \subcaptionbox{Step 32\label{subfig:gridCompfs13_spf_ux_E38}}
        {\includegraphics[scale=1,trim={0.7cm 10 0
              3},clip]{figures/ux_fs13_gridcomp_spf_E38.pdf}}
        \caption{Vertical velocity profiles for different step niches in
          the development region. Spillway flows with Froude number
          \textsf{F\textsubscript{s}}=13 and at different grids compared to
          physical model results by \cite{Bung2011}. }\label{fig:gridCompfs13_spf_ux}
\end{figure}


==> texfiles/spfluniformcomp.tex <==
%% The intention here is to compare against empirical formulations
% -Cmean, h90, hw(?)
% -uniform region -- onset, verify that the flow reaches uniform conditions
\subsection{Uniform region} % might change this heading

\begin{table}[htp]
  \caption{Depth averaged air concentration found by
    \ttt{spillwayFlow} (SPF) simulations compared to empirical expressions and
    physical model results by \cite{Bung2011}.}
  \label{tab:spfCmean}
  \begin{tabular}{llllll} %{ccccccc} %{llllll}
    \textbf{\textsf{F\textsubscript{s}}} & $C_{au}^{\text{SPF,G4}}$ &
    $C_{au}^{\text{SPF,G3}}$ & $C_{au}^{\text{Boes}}$ &
    $C_{au}^{\text{Bung,emp}}$ & $C_{au}^{\text{Bung,exper}}$  \\ 
    \hline
    2.7  & 0.36 & 0.33 & 0.59 & 0.42 & $\approx$0.4  \\ % case 
    4.6  & 0.28 & 0.25 & 0.57 & 0.37 & $\approx$0.31 \\ % case 
    8.3  & 0.37* & 0.41* & 0.31 & 0.31 & $\approx$0.24 \\ % case 
    13   & 0.26* & 0.30* & 0.53 & 0.26 & $\approx$0.23 \\ % case
    \hline
  \end{tabular}
\end{table}


%%%% Depth averaged alpha
%% Could perhaps made this as one plot - have to think about this...
%% dx=0.005
\begin{figure}[htp]
  \vspace{-10pt}
   \centering
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 20 0 0},clip]{figures/cmeanFigs/nedge_cmeanComp_fs27.pdf}
        \caption{\textsf{F\textsubscript{s}}=2.7}
        \label{subfig:h90_fs27_dx005}
    \end{subfigure}
    %% \bigskip
    \par\medskip
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 20 0 20},clip]{figures/cmeanFigs/nedge_cmeanComp_fs46_noLegend.pdf}
        \caption{\textsf{F\textsubscript{s}}=4.6}
        \label{subfig:h90_fs46_dx005}
    \end{subfigure}
    \par\medskip
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 20 0 20},clip]{figures/cmeanFigs/nedge_cmeanComp_fs82_noLegend.pdf}
        \caption{\textsf{F\textsubscript{s}}=8.28}
        \label{subfig:h90_fs82_dx005}
    \end{subfigure}
    \par\medskip
        \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=1,trim={0 10 0 20},clip]{figures/cmeanFigs/nedge_cmeanComp_fs13_noLegend.pdf}
        \caption{\textsf{F\textsubscript{s}}=13}
        \label{subfig:h90_fs13_dx005}
    \end{subfigure}
    \caption{Depth averaged void fraction. Spillway flows with different Froude
      numbers on the finest grid ($\Delta x=0.000625$ m, $\approx 5-7$ million
      cells) compared to physical model results by
      \cite{Bung2011}, and an empirical relation by
      \cite{Pfister2011}.}\label{fig:h90_fscomp_dx005}  
\end{figure}

